Attacks and Defenses for Free-Riders in Multi-Discriminator GAN

Generative Adversarial Networks (GANs) are increasingly adopted by the industry to synthesize realistic images. Due to data not being centrally available, Multi-Discriminator (MD)-GANs training framework employs multiple discriminators that have direct access to the real data. Distributedly training a joint GAN model entails the risk of free-riders, i.e., participants that aim to benefit from the common model while only pretending to participate in the training process. In this paper, we conduct the first characterization study of the impact of free-riders on MD-GAN. Based on two production prototypes of MD-GAN, we find that free-riders drastically reduce the ability of MD-GANs to produce images that are indistinguishable from real data, i.e., they increase the FID score -- the standard measure to assess the quality of generated images. To mitigate the model degradation, we propose a defense strategy against free-riders in MD-GAN, termed DFG. DFG distinguishes free-riders and benign participants through periodic probing and clustering of discriminators' responses based on a reference response of free-riders, which then allows the generator to exclude the detected free-riders from the training. Furthermore, we extend our defense, termed DFG+, to enable discriminators to filter out free-riders at the variant of MD-GAN that allows peer exchanges of discriminators networks. Extensive evaluation on various scenarios of free-riders, MD-GAN architecture, and three datasets show that our defenses effectively detect free-riders. With 1 to 5 free-riders, DFG and DFG+ averagely decreases FID by 5.22% to 11.53% for CIFAR10 and 5.79% to 13.22% for CIFAR100 in comparison to an attack without defense. In a shell, the proposed DFG(+) can effectively defend against free-riders without affecting benign clients at a negligible computation overhead.

==> section/assumption.tex <==
\section{Assumption of System}
\subsection{Assumptions of experiments}
1. Each client can know the model parameters of generator on demand. Because in the end, all participants want the generator.
2. Each participant has authentic data (except attackers), otherwise it cannot train discriminator.

\csr{what does the attacker see on the network? What can they impact, e.g., only their own behavior, or can they e.g., interrupt others? Given that it is a freerider attack, I assume they only can change their own behavior and they do not monitor the network?}

\subsection{Training details}
For the basic setting of experiment. Our framework contains 1 generator and N discriminators. Generator is in server side, each discriminator is in client side. For each round of training, if it is in the training phase for discriminator, each client trains its discriminator locally using its local data. During the training phase for generator, each discriminator will generate gradients for the generated data from generator. Then all the gradients will be used together (not one by one, this is important! If it's one by one, then the generator at time t and t+1 will be different, but all the gradients are calculated at time t.) to update generator \csr{how exactly are the 3 combined?}. And for three training methods, they have their own unique strategy to update.
\csr{how is the system initialized? how do clients decide to stop training (e.g., fixed number of rounds)? you only mention the training phase, are there other phases?}
\begin{itemize}
\item \textbf{\mdsimple} In this case (It's the same setting as in AsynDGAN, GMAN.), each client just train their discriminator using their local data. \csr{is there any other info they get? model parameters? model from previous round?}
\item \textbf{\mdswap} In this case (It's the same setting as in MD-GAN with aggregation weights), in the end of each epoch \csr{difference between rounds and epochs?}, each discriminator will swap the local model with another client in a p2p way.\csr{how is the other client selected? is it publicly known who swaps with whom?}
\item \textbf{\mdswitch} In this case (It's the same setting as in TDGAN), in the end of each epoch, there will be some randomness \csr{is what sense?} on the state of all the clients. Some of them can be off-line in the next epoch. Only online client can join the training for next epoch. And there is no swapping of the models. \csr{so it's like \textbf{\mdsimple} but with consideration for offline clients?}

\end{itemize}


\subsection{Expected experiments}
(1). 3 MDGAN frameworks, comparisons (i) with, (ii) without free-riders and (iii) with free-riders \& defense. 4 benign participants and 1 attack. 3 tabular datasets  and 1 image (MNIST) data.

Figures show for only one dataset, tables show results for all the datasets.
(2) time analysis for defense strategy.

==> section/characterizing.tex <==
\section{Free-riders in MDGAN}
\subsection{Experimental Setups}

